How Software Developers Mitigate Collaboration Friction with Chatbots

Modern software developers rely on an extensive set of social media tools and communication channels. The adoption of team communication platforms has led to the emergence of conversation-based tools and integrations, many of which are chatbots. Understanding how software developers manage their complex constellation of collaborators in conjunction with the practices and tools they use can bring valuable insights into socio-technical collaborative work in software development and other knowledge work domains. In this paper, we explore how chatbots can help reduce the friction points software developers face when working collaboratively. Using a socio-technical model for collaborative work, we identify three main areas for conflict: friction stemming from team interactions with each other, an individual's interactions with technology, and team interactions with technology. Finally, we provide a set of open questions for discussion within the research community.

==> sections/discussion.tex <==
%!TEX root = ../CSCW17-WorkshopPaper.tex

\section{Discussion}

% Productivity, as defined by Scacchi et al., includes the reduction of friction points [ref].
As Erik Raymond stated, "every good work of software starts by scratching a developer's personal itch" [cite cathedral bazaar paper].
This mindset, however, is reminiscent of the the early days of CSCW, when researchers focused on designing tools to support collaboration instead of understanding the collaborative practices themselves[ref needed?].
It can be argued that we shouldn't simply be throwing tools, or chatbots, at the issue, but rather understanding why developers need these tools.
Friction points that developers are identifying, and trying to self-medicate with chatbots, can provide valuable insights into the team's collaborative needs.

An early approach to examining the collaborative process in software development was Ellis's et al. \textbf{3C model}, which focuses on the interactions between \textit{communication}, conversations between developers; \textit{coordination}, dealing with conflicts; and \textit{collaboration}, working on tasks [ref needed]. In this paper we considered how chatbots support collaboration as a whole, but how do each of these bots support the communication and coordinate dimensions of the model?
The model was later expanded Gerosa et al. to include awareness, "an understanding of the activities of others, which provides context for your own activity" \cite{Dourish:1992:ACS:143457.143468}.

Researchers have identified four types of awareness in software development: informal or presence awareness, teammates availability; group structural awareness, team members roles and teams' internal structure; workspace awareness, when artifacts where changed and who changed them; social awareness, the social structure of the team [ref]. 
These subgroups of awareness work together to help team members construct and maintain their situational awareness, an awareness of the elements in their immediate environments \cite{Calefato:2012:ASA:2663638.2663642}.

Chatbots like Convergely provide support for presence awareness by allowing developers configure an automated response for when they are away from their desks.


NEED EXAMPLE OF BOT FOR TYPES OF AWARENESS

Software development involves not only formal learning, but also dynamic informal learning or 'learning by experience' \cite{Arciniegas-Mendez:2017}.  
Since dynamic learning is such a crucial part of successful software development, Arciniegas-Mendez et al. identified that developers must understand how to regulate their learning and proposed the Model of Regulation for software engineering. 
The model is composed of three modes of regulation: self-regulation, managing one's own goal directed behaviours; co-regulation, regulating the behaviours of others; and shared-regulation, joint regulation of the teams behaviours \cite{Arciniegas-Mendez:2017}.

Acebot\footnote{http://acebot.ai/}, for example, is an AI task management chatbot that supports self-, co-, and shared-regulation \cite{Arciniegas-Mendez:2017}.
Acebot supports self-regulation through viewing a list of your remaining and completed tasks, or by creating a to-do for yourself.  
Acebot supports co-regulation by looking at a subset of to-dos matching a specific keyword, or by creating and assigning to-dos to team members.
Acebot supports shared regulation through viewing the entire to-do list or completed tasks, or by creating open to-do tasks for the entire team.

Another question is whether there are any collaborative friction points or developer needs, that chatbots currently can not solve? Are there any needs that they will never be able to fill?

Perhaps the study of the chatbots themselves can also provide insights, and for this reason require further examination.
For the scope of this paper, we focused our attention of the subcategory of bots, chatbots.
A step towards studying the use of bots was Storey's et al. definition of 5 bot dimensions: how autonomous, how intelligent, how do they interact, how are they created, where do they reside, and what do they do \cite{Storey:2016:DDP:2950290.2983989}? 
They stressed the importance for examining how the use of bots by developers benefits developers in terms of productivity and project quality, and proposed a two dimensional productivity framework for studying bots: efficiency, supporting developers doing things faster; and effectiveness, helping developers move towards meaningful goals. With the effectiveness dimension, they explore how bots support collaboration efforts through the support of team cognition, regulation, and enhance decision making.


% talk about things that you didn't try to support
% talk about the other side of the the point
% - any area that they could never solve
% - any areas that they cant currently solve
% - focused purely on chatbot in the paper, but other bots may also support collaboration.
% - Are chatbots the right way to go?
% - Better ways to integrate chatbots in the developers workflow -- speech? IDE? Slack channel? 


==> sections/old_sections.tex <==
\section{Introduction}
\carly{this needs to be simplified, reduced, and made more motivational}

Software Development has rapidly transitioned from a solo activity, to a distributed collaborative activity that requires developer to keep up to date on many projects.  
Each of which may also have their own set of tools [hub \& spokes], impacting how developers work together and learn.
The use of many channels leads to information fragmentation, software artifacts generated becoming spread across many tools \cite{Storey:2012:ESP:2664446.2664469}.
For these reasons, many projects are adopting team communication and collaboration tools, such as Slack\footnote{https://www.slack.com}, Hipchat\footnote{https://www.hipchat.com}, Microsoft Teams\footnote{https://teams.microsoft.com}, Flowdock\footnote{https://www.flowdock.com/}. 

Although distributed software team might rely on these team messaging platforms for the bulk of their team communication, collocated teams can benefit from the use of such systems [find MS citation].  
These IRC-like tools provide a fully searchable interface consisting of persistent chat rooms, private group messages, and direct messages.

The widespread adoption of these team based platforms is a breeding ground for new, conversational based tools and integrations.
Among the intergeneration that can be supported are bots -- chatbots are a subgroup of bots that add and conversational interface onto the services. 
Although some bots have been around for years, the ease of integration of chatbots into modern communication tools has created and explosion of new chatbots recently.
Chatbots are services, usually powered by rules, machine learning, or artificial intelligence (AI), with which the user interacts via a conversational interface.
These conversational interfaces can include text input in a messaging system or spoken words.
MyVoiceBot\footnote{http://demo.softserveinc.com/voicemybot/} connects Amazon's Alexa\footnote{https://developer.amazon.com/alexa} to Hipchat, giving the user voice control over the normal text based interactions that they have with chatbots (configure specific updates, commands, etc).

Developers have been adopting these bots at a dizzying pace to fill many of the roles of that software developers have traditionally filled: maintaining code quality, preforming testing, conducting development operations, supporting customers, and constructing documentation \cite{Storey:2016:DDP:2950290.2983989}. 
However, little research has been conducted studying the impact that these bots have on software development efforts. 
How can we determine which ones will benefit teams in terms?

One step towards studying the use of chatbots was the definition of bot dimensions prosed by Storey et al. \cite{Storey:2016:DDP:2950290.2983989}. They identified that bots can differ across 5 bot dimensions: how \textit{autonomous}, how \textit{intelligent}, how do they \textit{interact}, how are they \textit{created}, where do they \textit{reside}, and what do they \textit{do}? They stressed the importance for examining how the use of bots by developers benefits developers in terms of productivity and project quality \cite{Storey:2016:DDP:2950290.2983989}. 
They propose studying bots on two main dimensions: \textit{efficiency}, supporting developers doing things faster; and \textit{effectiveness}, helping developers move towards meaningful goals.

Incorporate... 
\begin{itemize}
  \item more focus on collaboration -> team awareness -> learning -> regulation
  \item Platforms like slack make it easy for developers to create custom tools to support their needs -- way less overhead than their has been in the past
  \item Developers are already using tools like slack, so provide the collaboration support where they already are... or sync it with voice to they don't need to switch tasks when developing -- reduce distractions / overhead
  \item these tools are available on phones, tablets, desktops, so they can be in the loop when they aren't sitting at their desks.
\end{itemize}

In this short paper we propose the use of chatbots to aid developers in their collaborative efforts.
In the following, we introduce the model of regulation and give examples of how chatbots can be used to help facilitate the regulatory processes. 
In the next section, we provide recommendations on applying chatbot-power to software projects.  
This is followed by a discussion identifying possible risks and challenges associated with the use of \textit{chatbot-power}.

\section{Collaboration in Software Engineering}
\carly{more of a transition is needed here... fix the 3C, awareness, regulation issue}

One of the first approaches to examining the collaborative process in software development was the 3C model.
The 3C model examines the interactions between \textit{communication}, conversations between developers; \textit{coordination}, dealing with conflicts; and \textit{collaboration}, working on tasks. 
The 3C dimensions work together to promote group \textit{awareness}, which in turn mediates coordination, communication, and collaboration.

\subsection{The Model of Regulation}
The Model of Regulation for software development, prosed by Arciniegas-Mendez et al., is composed of three modes of regulation: self-regulation, co-regulation and shared-regulation \cite{Arciniegas-Mendez:2015,Arciniegas-Mendez:2017}.

\textbf{Self-regulation} refers to an "\textit{individual's} processes with respect to a task".
Self-regulation is a requirement in a collaborative setting, as it is need for the individual to manage their own thoughts, behaviors, and feelings towards reaching a goal.

\textbf{Co-regulation }is the outcome of individuals regulating the the behaviors of others.  
Co-regulation represents the beginning of alignment between the individual and group perspectives.

\textbf{Shared-regulation} is achieved when the group members' understanding aligns into a single group vision.  
Decisions made at this state effect the group as a whole, through joint control of the task.

Developers already use slack for personal, team-wise, and community wide communication ('slacking off paper') -> aligns well with self-, co-, and shared-regulation.     

Next, we examine how tools, particularly chatbots, can be used to help support 


\section{Chatbot Regulation Support }
The Model of Regulation propose by Arciniegas-Mendez et al. \cite{Arciniegas-Mendez:2015} describes four categories of tools supporting regulation: structuring support, mirroring support, awareness tools, and guiding systems.  
These tools can be used to support self-regulation, co-regulation, and shared-regulation depending on how the tool features are used and may provide a variety of regulation support. In the following, we give examples of how chatbots can be used to provide support for regulation within software development.


\textbf{Structuring support}
tools help users \textit{define} the roles and scripts used guide self-regulation interactions. 
\textit{Roles} represent the basic job functions or duties of team members.  
\textit{Scripts} represent the rules or processes that all team members agree to follow when completing larger tasks on the project.  
Chatbots can act as a self-regulatory structuring support tool by providing \textit{prompts} to the team members. 
These prompts are hints or suggestions, that help guide the user in taking the correct sequence of actions when completing tasks.

An example of a chatbot capable of providing structuring support is Slackbot\footnote{https://\foomy.slack.com/customize/slackbot}. 
Slackbot lives in the Slack platform, and works in the pull based manor. 
A team at a large software company employed Slackbot to help new team members get used to the projects scripts for completing tasks, such as merging their branches with production code. 
If the team members forgot the correct sequence of steps, they can trigger Slackbot using a word or phrase and have it respond with the predefined script.  
This saved them from not only interrupting other developers with repetitive questions, but also insured everyone was following the same procedures. 
This simple script could be enhanced to watch for certain behaviors, and send notifications to work in a more proactive manor.

Other examples of Chatbots providing structuring support are: DriftBot\footnote{https://www.drift.com/slack/}, helps directing customers to the correct team members who can help them with their issues; and Google Calendar\footnote{https://slack.com/apps/A0F8149ED-google-calendar}, a chatbot that reminds team members of upcoming meeting or other events. 

\textbf{Mirroring support}
tools help team members \textit{reflect} on the individual or collective actions that they have taken.  
Mirroring tools can help support self-regulation by providing the user feedback on their own actions, co-regulation by providing feedback on a subset of the team, or shared-regulation by providing feedback for the entire team.  

Acebot\footnote{http://acebot.ai/} is an AI task management chatbot that helps teams by providing mirroring support.
Acebot supports self-regulation through viewing a list of your to-dos / completed tasks, or by creating a to-do for yourself.  
Acebot supports co-regulation by looking at a subset of to-dos matching a specific keyword, or by creating and assigning to-dos to team members.
Acebot supports shared regulation through viewing the entire to-do list or completed tasks, or by creating open to-do tasks for the entire team.

Other chatbots that provide mirroring support include: TimeDoctor\footnote{https://www.timedoctor.com/}, a chatbot that supports self-regulation by summarizing time spent on each commit; SlackDigest\footnote{https://slackdigest.com/}, a chatbot that supports shared-regulation by creating daily summaries of Slack channels that the user has subscribed to; and WorkingOn\footnote{https://www.workingon.co/integrations/slack}, a chatbot that supports shared-regulation by allowing team members to give real time status updates.

% tools like trello, and github let you know when task have been added or moved around.

\textbf{Awareness support}
tools allow for team members to \textit{compare} their progress against their past performance or the performance of other team members. 
The key difference between mirroring and awareness support, is that in awareness support you can determine who completed which tasks.
Depending on if the information presented is for a small set of members or the entire group, the chatbot can support co-regulation or shared-regulation, respectively.

A potential awareness supporting chatbot could provide users with a summary or visualization of the commits made by themselves (self-regulation), a subgroup of team members (co-regulation), or the entire team (shared-regulation).

Other chatbots that provide awareness support include: Engineering Health Checker\footnote{https://svenpet.com/2015/11/30}, a virtual 'wall of shame' of developers who recently introduced heath issues in the code could be adapted into a chatbot supporting shared-regulation; Screenfully\footnote{http://screenful.com/guide/slack-integration/}, a shared-regulation supporting chatbot that shows completed tasks, ongoing tasks, and visualizations of the team's performance; and Jell\footnote{https://jell.com/slack}, a shared-regulation supporting chatbot that shares team member's accomplishments, ongoing tasks, and any blockers that they might be facing.

%screenfully / jell might fall more under mirroring, since you can't "compare" very easily

\textbf{Guiding support}
systems act as a virtual presence in the teams, monitoring and analyzing data so they can \textit{intervene} when collaboration issues are detected. 
With recent advances in natural language processing, machine learning, and artificial intelligence, there is a great potential for the use of chatbots in guiding collaboration.

Solid\footnote{https://getsolid.io/slackbot/} is a chatbot that provides guiding support for team meetings. Prior to the meetings commensing, Solid sends out reminders including the agenda, and lets you know if the meeting is not solid enough to be held.  During the meeting Solid will keep track of time remaining and any incomplete tasks.  After the meeting Solid sends team members a list of the outcome and tasks they are responsible for, along with a survey to determine the efficiency of the meeting.

Other examples of chatbots that provide guiding support include: Zeal's Ava Bot\footnote{https://slack.com/apps/A140633RA-zeals-ava-bot} and Mink\footnote{https://slack.com/apps/A1J8C37NG-mink}, shared-regulation supporting chatbots that provide team moral monitoring and raise issues to management when appropriate; Worklife\footnote{https://slack.com/apps/A0611JQAF-worklife-meeting-assistant}, a self-regulation (?) supporting meeting assistant that sends you snapshots of daily schedule, reminders of your meetings, allows you to add agenda items, and take collaborative notes during the meeting; To-Do bot, a self-regulation supporting chatbot that sends you reminders for upcoming task that haven't been started yet; and Tomatobot\footnote{https://slack.com/apps/A0QMVCPAR-tomatobot}, a self-regulation chatbot that tells you when it's time to take a break and allows you to record distractions to you can forget about them until your next break.

% Flaky Test Detector??


\section{Adopting Chatbots into Project Workflow}

%Through identifying collaboration, coordination, communication, awareness, and regulation friction points teams can start to get an idea of which types of chatbots they need. 
Since there are so many chatbots out there, to reduce the risk of tool overload what approach should teams take in determining which chatbots to integrate into their projects to provide the best support for team regulation?  
We adapted the \textit{recommendations for practitioners choosing tools} \cite{Storey:2012:ESP:2664446.2664469}, to provide a set of \textit{guidelines for adopting chatbots} into software development projects.

\carly{Taken right out of the paper, these need to be refining \& twisting to make them work for chatbots...}
\begin{itemize}
  \item beware of channel affordances, and choose tools accordingly
    \begin{itemize}
      \item when integrating chatbots into the project, developers need to consider the channel they have selected affordances.  
      \item For example, will the chatbot live on private / public channels / whole site, or all of the above?  
      \item Will the chatbot work in a pull based manor or interrupt when needed?  
      \item Will the chatbot interactions be synchronous or asynchronous? 
      \item Will the user be able to interact with the bot via voice or purely through text? 
    \end{itemize}
  \item Define a "communication covenant"
    \begin{itemize}
      \item Define which chatbots should be used to support which types of activities
      \item Define what to do when a chatbot is no longer working for it's intended purpose? adapt, modify, remove?
      \item Evaluate the chatbot in the social context of the team
      \item How to use the chatbots in an agreed upon way?
    \end{itemize}
  \item "Think lean"
    \begin{itemize}
      \item The chatbots should help reduce channel overload, not contribute to it.
      \item Start with a few chatbots that address the largest communication issues, and include more once users are used to them
      \item Adopt approaches like the hub and spokes model -- aggregate 
    \end{itemize}
  \item "Latest Tools"
    \begin{itemize}
      \item New bots are being developed every day that might help team communication process
      \item Many tools such as BeepBoop\footnote{https://beepboophq.com/} make it easy to create custom bots, for multiple platforms with very little overhead.
    \end{itemize}
  \item "Learn" how to use the channels most effectively
    \begin{itemize}
      \item Incorporating chatbots into your team will be of little use if know one learns how to effectively use them to promote awareness, communication within the team
      \item tool literacy is extremely important, as when it is lacking it can lead to frustration which might worsen the communication issues
    \end{itemize}
  \item Allow developers to unplug
    \begin{itemize}
      \item showed and example of a chatbot to allow developers to reduce distractions / interruptions?
      \item developers should be able to control which chatbots they allow to interact with them, when they are allowed to, and when they need some personal time.
    \end{itemize}
\end{itemize}

\section{Risks and Challenges}

Little is known about the use of bot for software development.  
% Storey and Zagalsky stress the importance for examining how the use of bots by developers benefits developers in terms of productivity and project quality \cite{Storey:2016:DDP:2950290.2983989}. 
% They propose studying bots on two main dimensions: \textit{efficiency}, supporting developers doing things faster; and \textit{effectiveness}, helping developers move towards meaningful goals.

However, there are many other considerations when using bots:
\begin{itemize}
  \item{Will adding these bots into our workflow change the ways that developers work with each other? Interact with each other? Relate to each other?
  For better or worse?}
  \item{Will adding bot-power have other, unexpected outcomes? Ie. slow down the project, create new friction points, ...}
  \item{Could using bots to support regulation, actually hamper the user's ability to self-regulate without the use of bots / prompts?  How much is too much offloading?}
  \item{What if the bots go rogue?}
  \item{Some actions aren't discoverable, but on the other hand -- people may think they are capable of more than they are.}
  \item{Ethics for using the bots -- when do we know we've crossed the line?}
\end{itemize}

\section{Discussion and Future Work}

- for the scope of this paper, we focused on chatbots that directly supported self-, co-, and shared-regulation. There are likely other chatbots, or even bots, that help indirectly facilitate these processes.
- Are chatbots the right way to go?
- Better ways to integrate chatbots in the developers workflow -- speech? IDE? Slack channel? 



==> sections/risks_challenges.tex <==
%!TEX root = ../CSCW17-WorkshopPaper.tex

\section{Risks \& Challenges}

Developers are rapidly embracing these chatty virtual team members into their software development projects.  
However, are developers stopping to take the time to think about the true cost of adding these chatbots to the team?  

Research has shown that the ways we interact with technology, changes the way the we interact with each other [ref]. 
Will adding chatbots into our collaborative processes change the ways that developers interact or collaborate with each other?  
Will these changes be for better or for worse?
Will having chatbots facilitate processes for developers, such as regulation \cite{Arciniegas-Mendez:2017}, hamper the users ability to preform these processes for themselves?

In software development, it is often considered bad practice to be to reliant on external services.  
What are the risks involved in relying on chatbots to facilitate one of the most essential aspects of a successful software development project, collaboration?

According to Brookes Law "adding manpower to a late software project makes it later" \cite{Brooks:1995:MM:207583}. Would adding chatbots to a late project make it even later?

Team specific configuration is also needed for even the most simple of chatbots.  
The more complex bots, or ones the teams build for themselves often require training to before they reach their full potential.
Like a new developer entering the team, the chatbot has to be taught the ins and outs of the processes they will be automating.

Existing team members need to be introduced to the new chatbot, and learn how it will fit into their development processes.
Developers may have to spend time bringing themselves back to the same level they were working at, prior to the introduction of the chatbot. The more disruptive the change is to the developer's workflow, the longer it would take to return to the same productivity level as before.

[Ethics for using the bots -- when do we know we've crossed the line?]


% Could adding chatbots to a software project have other possible side effects that we have yet to consider?  

% Currently, AI technologies can quickly deteriorate when faced with unexpected inputs. A recent example of this is Microsoft's Tay bot\footnote{http://blogs.microsoft.com/blog/2016/03/25/learning-tays-introduction/}, a twitter chatbot who began posting discriminatory and insensitive tweets.  As AI continues to become more powerful, what do we risk to lose?

% Some actions aren't discoverable, but on the other hand -- people may think they are capable of more than they are.

% Would the end users of the software comfortable knowing that chatbots helped build the software that they are using?

